Fat Pointers for Temporal Memory Safety of C

Temporal memory safety bugs, especially use-after-free and double free bugs, pose a major security threat to C programs. Real-world exploits utilizing these bugs enable attackers to read and write arbitrary memory locations, causing disastrous violations of confidentiality, integrity, and availability. Many previous solutions retrofit temporal memory safety to C, but they all either incur high performance overhead and/or miss detecting certain types of temporal memory safety bugs. In this paper, we propose a temporal memory safety solution that is both efficient and comprehensive. Specifically, we extend Checked C, a spatially-safe extension to C, with temporally-safe pointers. These are implemented by combining two techniques: fat pointers and dynamic key-lock checks. We show that the fat-pointer solution significantly improves running time and memory overhead compared to the disjoint-metadata approach that provides the same level of protection. With empirical program data and hands-on experience porting real-world applications, we also show that our solution is practical in terms of backward compatibility -- one of the major complaints about fat pointers.

==> Makefile <==
TARGET=checkedc

LATEX=pdflatex
BIBTEX=bibtex
TEXFILES = $(wildcard *.tex) $(wildcard tables/*.tex) $(wildcard alg/*.tex)
CODEFILES = $(wildcard code/*.s)
BIBFILES = $(wildcard *.bib) $(wildcard ../../bibtex/*.bib)

FIGFILES = $(wildcard figs/*.pdf)
FIGFILES +=$(wildcard figs/*.tex) $(wildcard figs/*.pdf) $(wildcard figs/*.png)
CONFFILES += $(wildcard *.sty) $(wildcard *.cls)

.PRECIOUS: %.ps %.pdf

.PHONY: $(TARGET) clean clean-full

$(TARGET): $(TARGET).pdf

$(TARGET).pdf: $(TEXFILES) $(CODEFILES) $(FIGFILES) $(BIBFILES) $(CONFILES)
	-rm -f *.aux
	$(LATEX) $(TARGET).tex
	$(BIBTEX) $(TARGET)
	$(LATEX) $(TARGET).tex
	$(LATEX) $(TARGET).tex
	@/bin/echo ""
	@/bin/echo "++++++++++++++++++++++++++++++++++++++++++++++++++++++++++"
	@/bin/echo "               ++++ ANY UNDEFINED REFERENCES ++++"
	-@grep -i undef $(TARGET).log || echo "No undefined references."
	@/bin/echo "                 ++++ ANY EMPTY REFERENCES ++++"
	-@egrep -i -n -e 'cite{ *}' -e 'ref{ *}' $(TEXFILES) $(FIGFILES) || echo "No empty references."
	@/bin/echo "++++++++++++++++++++++++++++++++++++++++++++++++++++++++++"
	@/bin/echo ""

#
# Build a PDF without comment
# Only tested on a MacOS.
#
nc:
	@sed -i'.original' 's/% \\def\\Comment#1{}/\\def\\Comment#1{}/' $(TARGET).tex
	@make
	@sed -i'.nocomment' 's/\\def\\Comment#1{}/% \\def\\Comment#1{}/' $(TARGET).tex
	@rm -f $(TARGET).tex.original $(TARGET).tex.nocomment

clean:
	rm -f *.aux *.bbl *.dvi *.lof *.log *.toc *.lot *.blg *.out *._paper.pdf

clean-full: clean
	rm -f $(TARGET).pdf


==> discuss.tex <==
%==============================================================================%
\section{Discussions}
\label{section:discuss}
%==============================================================================%

%
% Discuss other potential design choices.
%

%------------------------------------------------------------------------------%
\subsection{Secure Languages vs. Compiler Instrumentations}
%------------------------------------------------------------------------------%
%
% - Readability of source code is important
% - Incremental conversion is important
% - Is safe implementation more error-prone?
% - PL does not care where a pointer (or any other data) lives, while safe
%   implementation needs to differentiate data in memory and registers.
%

%------------------------------------------------------------------------------%
\subsection{Compare with Rust's Model of Borrowing}
%------------------------------------------------------------------------------%


==> future.tex <==
%==============================================================================%
\section{Future Work}
\label{section:future}
%==============================================================================%

%
% Future works
%
%------------------------------------------------------------------------------%
\subsection{Support for 32-bit Systems}
\label{section:future:32}
%------------------------------------------------------------------------------%

%------------------------------------------------------------------------------%
\subsection{Multithreading Support}
\label{section:future:multithreading}
%------------------------------------------------------------------------------%


==> intro_new.tex <==
%==============================================================================%
\section{Introduction}
\label{section:intro}
%==============================================================================%

%
% Why no good solution for memory safety
%
Memory safety vulnerabilities are still a serious problem for C
programs~\cite{cvetrend,VulTrend:BlueHatIL19} despite decades of
research aiming to prevent
them~\cite{EternalWar:Oakland13,SanitizerSoK:Oakland19}.
Static analysis~\cite{BLinesOfCode:Coverity,Infer:FB} and fuzz
testing~\cite{FuzzingSurvey:IEEE,FuzzingSurvey:ITOSE19} can catch bugs
before code is shipped, but they miss vulnerabilities and suffer
scalability and/or usability issues. C code can be compiled to include
run-time safety checks~\cite{SafeC:PLDI94, CCured:TOPLAS05,ASan:ATC12,
SoftBoundCETS:SNAPL15,SanitizerSoK:Oakland19} but the added
overhead is a practical barrier to
deployment. Moreover, challenging code idioms may not be handled
soundly~\cite{ASan:ATC12,SoftBoundCETS:SNAPL15} or may cause the
compilation process to fail~\cite{CCured:TOPLAS05}.

%
% Why Safe C, Checked C?
%
One way to address these problems is to rewrite security-critical C code
in a memory-safe systems programming language such as
Rust~\cite{rustlang}. While doing so can be
efficacious~\cite{Tock:SOSP17,Servo:Mozilla}, it is labor intensive,
as Rust's allowed programming idioms are very different from
C, and automated conversion is (for now)
impractical~\cite{emre2021c2rust}.
%
Recently, \citet{CheckedC:SecDev18} proposed
{\CheckedC} as a spatially-memory safe target to which to convert legacy/active C
code. {\CheckedC} takes inspiration from prior work on
safe-C dialects~\cite{Cyclone:ATC02,ControlC:CASES02, Deputy:ESOP07},
but differs in that it includes
affordances, including a kind of \emph{gradual typing}~\cite{siek2007gradual},
to ease porting legacy code and
interoperating with it. {\CheckedC}'s performance is good:
\citet{CheckedC:SecDev18} reported average run-time overheads of
8.6\% on a small pointer-intensive benchmark suite,
and \citet{FreeBSDCheckedC:SecDev20} found
essentially no overhead when running {\CheckedC}-converted portions of
the FreeBSD kernel. By contrast, prior systems enforcing spatial
safety experienced overheads of between 60\%-200\%~\cite{CCured:TOPLAS05,
ASan:ATC12,SoftBound:PLDI09,SanitizerSoK:Oakland19}.

%
% Need temporal safety
%
As mentioned, {\CheckedC} currently focuses on
\emph{spatial safety} (i.e., avoiding buffer overflows), and provides
no support for \emph{temporal safety}. This is a significant limitation.
%
% A temporal memory safety violation occurs when
% a program dereferences a pointer whose referent has already been freed
% (\emph{use after free} or UAF), frees a pointer more than once (\emph{double free}),
% or frees a pointer that does not point to the start of a
% heap object (\emph{invalid free}).
An attacker may exploit temporal memory safety violations such
\emph{use-after-free} (UAF) and \emph{double free} bugs by using
a dangling pointer to read or write an arbitrary memory location,
inducing information leaks, memory corruption, or even arbitrary code
execution~\cite{UAF:CWE416,UAF:BlackHatUSA07,UAFKernel:CCS15,MallocMaleficarum}.
% Unfortunately, the past decade has seen an increase in such exploits
% used in the real world~\cite{ExploitTrend:MS13,
% VulTrend:BlueHatIL19,ChromeSecuritySurvey:2020}.
% MWH: Don't need this---should already have been covered in the first paragraph
Our work aims to remedy this weakness: We have developed an approach to
enforce temporal memory safety for {\CheckedC}, to complement its
spatial safety enforcement mechanisms.

An effective way to enforce temporal memory safety is to associate
each memory object with a distinct \emph{lock},
and each pointer with a \emph{key}. An object's lock is invalidated
when it is freed. At each pointer dereference, a dynamic check
confirms the pointer's key matches the referent object's lock;
if not, it signals a UAF\@.
While this basic
approach is popular in prior work~\cite{SafeC:PLDI94,Guarding:SPE97,CETS:ISMM10,
XuMemSafe:FSE04,UAFSan:ISSTA21,PTAuth:Sec21}, it tends
to incur high performance and memory overhead (e.g., 48\% on
selected SPEC CPU2006 benchmarks~\cite{CETS:ISMM10}).
% For example, CETS~\cite{CETS:ISMM10} incurs 48~\% performance overhead,
% and PTAuth~\cite{PTAuth:Sec21}---the latest work in this category---provides
% partial protection with 26~\% overhead
% for new ARM processors, both on selected SPEC CPU2006 benchmarks.
%
% Another way to mitigate temporal memory safety bugs is to invalidate
% dangling pointers at memory deallocation~\cite{DANGNULL:NDSS15,
% FreeSentry:NDSS15,DangSan:EuroSys17,HeapExpo:ACSAC20},
% but they are also slow (over 40~\% overhead without using extra CPU cores)
% and miss dangerous bugs~\cite{HeapExpo:ACSAC20}.
% Secure memory allocators are also explored to lower the possibility of
% reusing memory to mitigate UAF bugs~\cite{FreeBSDmalloc:EuroBSD09,
% DieHarder:CCS10,Cling:Sec10,FreeGuard:CCS17,Oscar:Sec17,FFmalloc:Sec21}.
% They can trade memory for performance and security, but the memory overhead
% can be prohibitive, and many of them are circumventable~\cite{DANGNULL:NDSS15}.
%
When experimenting with key-lock check approaches, we found that
a crucial reason for their high cost is
the use of \emph{disjoint} data structures, such as look-up tables,
to maintain the association between keys/locks and pointers/objects.
% MWH: Reads weird to me
% (this might be evident in retrospect, but to the best of our knowledge,
% we are the first to make this observation).
Doing so keeps objects and pointers unchanged from their legacy
representation, which makes it easy for compiled-to-be-safe code to
interoperate with unchanged (e.g., library) code. But the approach
requires many added instructions to locate the keys and locks at pointer
propagations and dereferences.

We observe that disjoint metadata is unnecessary when enforcing
temporal safety as a \emph{language feature} rather than a
\emph{compilation strategy}.  This is because representation
differences between safe and legacy pointers can be reflected in those
pointers' types, and programmers can choose when and how to convert
between them. This observation led us to explore the use of
\emph{in-place} metadata to represent pointer keys, as a kind of
\emph{fat pointer}.\footnote{Some works (e.g., \cite{SoftBoundCETS:SNAPL15})
refer to all techniques that
  associate pointers with metadata as fat pointers.  In this paper we
  use ``fat pointers'' to only mean pointers with in-place metadata.}
In particular, we extend {\CheckedC} with two new checked pointer
types, {\mmptrT} for pointers to single objects, and {\mmarrayptrT}
for pointers to arrays.\footnote{Two additional variants of these are
also available; see \secref{section:design:largeptr}.}
Values of these types are two machine words:
one word is the actual pointer, and the other word is the key plus necessary
metadata to locate the lock;
allocated objects are prepended with a lock (including stack-allocated
ones). We leverage {\CheckedC}'s \emph{inter-op types}~\cite{CheckedCTR:Microsoft}
to ease interfacing with legacy code.
% Though fat pointers fell out of favor for enforcing spatial
% memory safety~\cite{Cyclone:ATC02,CCured:POPL02}, our hope was that
% they could be significantly faster than the alternative when enforcing
% temporal safety.

% Fat pointers were oft-proposed for enforcing spatial memory
% safety~\cite{Cyclone:ATC02,CCured:POPL02} but fell out of
% favor because of both high overhead and difficulties interoperating
% with legacy components which assume the ``thin'' pointer representation.
% However, it is an open question whether fat pointers could be a
% practical solution to retrofit temporal memory safety to C.
% We observe that fat pointers could work in this role, under
% the current {\CheckedC} infrastructure.

% to enforce the key-lock check mechanism for temporal memory safety.
% Besides the performance benefit brought by in-place metadata
% and new safe pointers types,
% another key reason for our choice of this research direction
% is that {\CheckedC} grants programmers fine-grained low-level
% control over the source code and thus allowing manual intervention to solve
% backward compatibility issues caused by fat pointers,
% which is very challenging to achieve with pure compiler
% transformations~\cite{CCured:TOPLAS05,SoftBound:PLDI09}.

% \mwh{I don't really like this paragraph. I'd prefer a more straight-up
%   presentation: We implemented this approach in the Checked C
%   compiler, which is based on Clang/LLVM. As part of our
%   implementation, we developed optimizations xX and YY. We ported N
%   programs to use these pointers and measured their time and space
%   overhead. Etc. etc.}
% \mwh{Somewhere we should say that we have not yet completely
%   integrated into Checked C. That is, we are just confirming that it
%   can work, and that overhead is not too high. We'll integrate as a
%   next step.}
% \mwh{Also: Missing the related work forward reference}

% In this paper, we describe the design details of the new pointers
% (\secref{section:design}) and how we address the backward compatibility
% issues (\secref{section:compatibility}).
We implemented the new pointers in the Checked C compiler,
which is based on Clang/LLVM\@.
By design, these pointers extend {\CheckedC}'s spatially-safe pointers,
so in a full implementation they would be subject to spatial
safety checks. We have delayed this (straightforward, though nontrivial)
integration effort in order to first evaluate the effectiveness
of in-place metadata for temporal checking.\footnote{We describe the extensions
to {\CheckedC}'s spatially-safe pointers in Section~1 of
the supplementary material.\label{fullysafe}}
% We believe
% integration should be a straightforward (though substantial) effort
% \mwh{cite appendix}.
% One implementation limitation is that our prototype currently does not
% enforce spatial memory safety, although by design the new pointers extend
% {\CheckedC}'s spatially-memory-safe pointers.
% Making the temporally-safe pointers spatially safe would
% have required substantial additional engineering effort.
% Integrating spatial memory safety to our prototype is in the future work.
%
% We also briefly explain the implementation, including redundant
% key check optimization (\secref{section:impl}).
To do so,
we ported Olden (a small pointer-intensive benchmark suite) and three
real-world applications to use temporally safe pointers and measured
the resulting performance and memory overhead (\secref{section:eval}).
We compared our {\CheckedC} solution with CETS~\cite{CETS:ISMM10}---the
state-of-the-art key-lock check approach using disjoint metadata---and
show that our in-place mechanism significantly reduces
performance overhead (29\% vs. 92\%) and
memory overhead (72\% vs. 202\%) on Olden.
We also discuss and compare our work with other key-lock check approaches and
two other major types of temporal memory safety solutions:
dangling pointer invalidation~\cite{DANGNULL:NDSS15,FreeSentry:NDSS15,
DangSan:EuroSys17,HeapExpo:ACSAC20} and secure memory
allocators~\cite{FreeBSDmalloc:EuroBSD09,DieHarder:CCS10,
Cling:Sec10,FreeGuard:CCS17,Oscar:Sec17,FFmalloc:Sec21}
(\secref{section:related}).

% The new safe pointers provide comprehensive temporal memory safety guarantees
% (\textsection~\ref{section:design}) and enable the compiler
% to conduct optimizations more easily (\textsection~\ref{section:impl}).
% For backward compatibility, we show (with empirical program
% statistics) that our fat pointer solution is practical
% (\textsection~\ref{section:compatibility}).
% We evaluated the performance and memory overhead on Olden
% (a small pointer-intensive benchmark
% suite~\cite{Olden:TOPLAS95,CompilerPrefetch:ASPLOS96}) and three
% real-world applications (\textsection~\ref{section:eval}).
% Our {\CheckedC} solution significantly improves
% the performance (29~\% vs. 92~\%) and memory consumption (72~\% vs. 202~\%)
% on Olden compared with CETS~\cite{CETS:ISMM10}---the state-of-the-art
% key-lock check approach using disjoint metadata.
% Finally, we discuss two other major temporal memory safety solutions for
% C---dangling pointer invalidations and secure memory
% allocators---and compare our solution with them
% (\textsection~\ref{section:related}).

In summary, we make the following contributions:

\begin{itemize}
    \item We explore the benefits and costs of using fat pointers to
        retrofit temporal memory safety to C
        (\secref{section:design}). We show that our solution is
        practical in terms of backward compatibility with legacy C code
      (\secref{section:compatibility}).

    \item We extend {\CheckedC} with new types of safe pointers to detect
        temporal memory safety bugs.  We implemented the new pointers
        using the LLVM compiler infrastructure for 64-bit systems (\secref{section:impl}).

    \item We evaluated the new safe pointers by measuring their performance
        and memory overhead. We show that our fat pointer solution
        significantly lowers the performance and memory overhead compared
        to a state-of-the-art disjoint metadata mechanism (\secref{section:eval}).

      \item As far as we are aware, ours is the first full temporal
          memory safety approach for C \mwh{this is Checked C, not C} which uses only in-place metadata,
          and simultaneously accounts for backward compatibility.

\end{itemize}


==> tables/bugs.tex <==
% Rename the check and cross mark.
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\question}{\textbf{\textit{?}}}

\begin{table}[tb]
    \caption{Temporal Memory Safety Bugs.
    The last three columns lists whether a type of bug may affect a program in
    the following ways:
    information leak ({\bf C}onfidentiality), data corruption ({\bf I}ntegrity),
    and program crash or denial of service ({\bf A}vailibility).
    {\cmark} means a direct cause. {\question} means it may affect indirectly
    when combined with other attacks.}
\label{table:bugs}
\centering
{\sffamily
\footnotesize{
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllll}
    \toprule
    \multirow{2}{*}{\bf Bug} & \multirow{2}{*}{\bf Description} &
    \multicolumn{3}{c}{\bf Affect} \\
    & & {\bf C} & {\bf I} & {\bf A} \\
    \midrule
    use-after-free &  Dereference a ptr after it is freed. & \cmark & \cmark & \cmark \\
    double free & Free a ptr after it has been freed. & \question & \cmark & \cmark \\
    invalid free & Free a ptr not to the start of an obj. & \question & \cmark & \cmark \\
    \bottomrule
\end{tabular}
}}}
\end{table}


==> tables/lzfse_perf.tex <==
%
% Performance data about lzfse
%
\begin{table}[tb]
\caption{{\CheckedC} Performance Overhead on {\tt lzfse}}
\label{table:lzfse_perf}
\centering
{\sffamily
\footnotesize{
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lrrrcrr@{}}
\toprule
\multirow{3}{*}{{\bf Data}} &
\multirow{3}{*}{\bf Size} &
\multicolumn{2}{c}{{\bf Compress}} & \phantom{} &
\multicolumn{2}{c}{{\bf {Decompress}}} \\
& & \begin{tabular}{@{}l@{}} {\bf Baseline} \\ {\bf Rate} \end{tabular} &
	\begin{tabular}{@{}l@{}} {\bf Check-} \\ {\bf ed~C} \end{tabular} & &
	\begin{tabular}{@{}l@{}} {\bf Baseline} \\ {\bf Rate} \end{tabular} &
	\begin{tabular}{@{}l@{}} {\bf Check-} \\ {\bf ed~C} \end{tabular} \\
\midrule
dickens & 9.8~MB & 52.5~MB/s & 4.4\% & & 356.8~MB/s & 11.2\% \\
mozilla & 49~MB & 73.3~MB/s & 6.8\% & & 471.8~MB/s & 10.4\% \\
mr & 9.6~MB & 64.9~MB/s & 4.2\% & & 418.4~MB/s & 10.8\% \\
nci & 32~MB & 123.0~MB/s & 20.9\% & & 555.7~MB/s & 7.7\% \\
ooffice & 5.9~MB & 58.1~MB/s & 4.8\% & & 375.7~MB/s & 10.9\% \\
osdb & 9.7~MB & 71.7~MB/s & 5.4\% & & 551.0~MB/s & 9.5\% \\
reymont & 6.4~MB & 65.5~MB/s & 6.4\% & & 402.0~MB/s & 11.0\% \\
samba & 21~MB & 83.1~MB/s & 8.9\% & & 324.5~MB/s & 10.6\% \\
sao & 7.0~MB & 58.6~MB/s & 3.9\% & & 355.8~MB/s & 10.5\% \\
webster & 40~MB & 62.3~MB/s & 6.1\% & & 436.9~MB/s & 10.2\% \\
xml & 5.1~MB & 102.4~MB/s & 14.2\% & & 561.2~MB/s & 8.6\% \\
x-ray & 8.1~MB & 56.4~MB/s & 3.4\% & & 332.3~MB/s & 11.0\% \\
enwik9 & 954~MB & 62.1~MB/s & 5.5\% & & 437.2~MB/s & 10.5\% \\
\midrule
{\bf Min} & 5.1~MB & 52.5~MB/s & 3.4\% & & 324.5~MB/s & 7.7\% \\
{\bf Max} & 954~MB & 123.0~MB/s & 20.9\% & & 561.2~MB/s & 11.2\% \\
{\bf Geomean} & --- & --- & 7.4\% & &--- & 10.2\%\\
\bottomrule
\end{tabular}
}}}
\end{table}

==> tables/olden.tex <==
%
% Execution time of baseline Olden
%
\begin{table}[tb]
\centering
{\sffamily
\footnotesize{
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lllllllll}
    \toprule
    bh & bisort & em3d & health & mst & perimeter & power & treeadd & tsp \\
    \midrule
    10.41 & 18.62 & 10.04 & 5.38 & 6.72 & 1.97 & 0.35 & 1.43 & 12.63 \\
    \bottomrule
\end{tabular}
}}}
\caption{Execution Time (s) of Baseline Olden Benchmarks}
\label{table:olden}
\end{table}

